HF-Fed: Hierarchical based customized Federated Learning Framework for X-Ray Imaging

In clinical applications, X-ray technology is vital for noninvasive examinations like mammography, providing essential anatomical information. However, the radiation risk associated with X-ray procedures raises concerns. X-ray reconstruction is crucial in medical imaging for detailed visual representations of internal structures, aiding diagnosis and treatment without invasive procedures. Recent advancements in deep learning (DL) have shown promise in X-ray reconstruction, but conventional DL methods often require centralized aggregation of large datasets, leading to domain shifts and privacy issues. To address these challenges, we introduce the Hierarchical Framework-based Federated Learning method (HF-Fed) for customized X-ray imaging. HF-Fed tackles X-ray imaging optimization by decomposing the problem into local data adaptation and holistic X-ray imaging. It employs a hospital-specific hierarchical framework and a shared common imaging network called Network of Networks (NoN) to acquire stable features from diverse data distributions. The hierarchical hypernetwork extracts domain-specific hyperparameters, conditioning the NoN for customized X-ray reconstruction. Experimental results demonstrate HF-Fed's competitive performance, offering a promising solution for enhancing X-ray imaging without data sharing. This study significantly contributes to the literature on federated learning in healthcare, providing valuable insights for policymakers and healthcare providers. The source code and pre-trained HF-Fed model are available at \url{https://tisharepo.github.io/Webpage/}.

==> algorithm.tex <==
\begin{figure*}[t]
\centering
\hspace{-5em}
\begin{minipage}[b][7.5cm][t]{0.60\linewidth} 
\begin{algorithm}[H]
%  \hfill
\caption{Mask Annealing updating process}
\label{alg:adversarial_training}
\tiny
\begin{algorithmic}[1]
    \State \textbf{Input:} weight parameters ($\theta_T$), masking ratio ($\mu_t$), step ($\eta$), warm restart epoch ($T_{\text{i}})$, max epochs ($T_{\text{max}})$, epochs since last restart ($T_{\text{c}})$, ranges for the steps ($\eta^i_{\text{min}}$, $\eta^i_{\text{max}}$)
    \State \textbf{Data:} $b_{\text{st}} = \{(x^s_{i})\}_{i=1}^{N_s} \cup \{x^t_{j}\}_{j=1}^{N_t}$\hfill \textit{\Comment{Batch}}
    \State Initialize hyperparameters: $\mu = 0.3$, step $\eta = 0.01$, batch size $b = 16$, max epochs $T_{\text{max}} = 40$, initializing parameters of network $\theta_T$ using source trained parameters.
    
    \For{$i$ in $1$ to $T_{\text{max}}$}
        \State $\eta_t = \eta^i_{\text{min}} + \frac{1}{2}(\eta - \eta^i_{\text{min}}) \left(1 + \cos\left(\frac{T_{\text{c}}}{T_{\text{i}}}\pi\right)\right)$\hfill\textit{cosine annealing}
        
        \State  $L = \mathcal{L}_{\text{mask}}(b_{\text{st}}, \theta_T)$ \hfill \textit{\Comment{Computing loss for batch $b_{st}$}}

        \State  $\nabla_{\theta} L = \nabla_{\theta}f_t(b_{\text{st}}, \theta_T)$ \hfill \textit{\Comment{Computing gradients}}
        
        \State  $\theta_T' = \theta_T - \eta_t \cdot \nabla_{\theta} L$ \hfill \textit{\Comment{Updating parameters}}

       \State  $\mu = \mu + \eta_t$ if $L < \bar{L}$, otherwise $\mu = \mu - \eta_t$ \hfill \textit{\Comment{Updating $\mu$}}
        
        \State  $i = i + 1$ \hfill \textit{\Comment{Incrementing epoch}}
    \EndFor
    \State \textbf{Return} parameters $\theta_T'$, $\mu'$.
\end{algorithmic}
\end{algorithm}
\end{minipage}
\hspace{0.15em}
\begin{minipage}[b][6.7 cm][t]{0.22\linewidth} % Adjust the height as needed
  \centering
   % \hspace{-1.05em}
  % \vspace{0.11 cm}
  \includegraphics[height=5.0cm]{Images/flow.pdf} \\
  \label{fig:figure1and2}
    % \vspace{-0.3 cm}
\end{minipage}
\vspace{-3.5em}
\caption{Mask Annealing Algorithm \textbf{(left)} and Adaptive Confidence Refinement \textbf{(right)} flowchart depicts the gradual transition of confidence threshold from soft to hard.}
\label{algo}
\end{figure*}


==> tables/fig1.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.18\textwidth} % Adjust the width of each subfigure
        \centering
        \includegraphics[width=\textwidth, height=3cm]{Images/fp1.png}
        \subcaption{}
        \label{f1a}
    \end{subfigure} % Remove the gap between subfigures
    \begin{subfigure}[b]{0.18\textwidth} % Adjust the width of each subfigure
        \centering
        \includegraphics[width=\textwidth, height=3cm]{Images/fp2.png}
        \subcaption{}
        \label{f1b}
    \end{subfigure}\hfill % Remove the gap between subfigures
    \begin{subfigure}[b]{0.6\textwidth} % Adjust the width of each subfigure
        \centering
        \hspace{-0.8 cm}
        \includegraphics[width=\textwidth, height=3cm]{Images/uda.pdf}
        \subcaption{}
        \label{f1c}
    \end{subfigure}
    \caption{(a) and (b) depict false positive predictions by current teacher student models in cross-domain \bcdm. Red boxes indicate ground truth, yellow boxes show MRT \cite{zhao2023masked} predictions, and green boxes indicate predictions from \myname. As shown in (c), our approach effectively mitigates the domain gap and makes accurate predictions.}
    \label{fig:all}
\end{figure}

==> tables/fig2.tex <==
\begin{figure}[t]
    \centering
    % \begin{subfigure}[t]{0.155\textwidth}
    %     \includegraphics[width=\textwidth, height = 2.5 cm]{Images/gt2.png}
    %     % No caption for Image 5
        
    % \end{subfigure}
    % \begin{subfigure}[t]{0.155\textwidth}
    %     \includegraphics[width=\textwidth, height=2.5 cm]{Images/sourceonly2.png}
    %     % No caption for Image 1
      
    % \end{subfigure}
    % \begin{subfigure}[t]{0.155\textwidth}
    %     \includegraphics[width=\textwidth, height=2.5 cm]{Images/at.png}
    %     % No caption for Image 2
        
    % \end{subfigure}
    % \begin{subfigure}[t]{0.155\textwidth}
    %     \includegraphics[width=\textwidth, height = 2.5 cm]{Images/bs2.png}
    %     % No caption for Image 5
        
    % \end{subfigure}
    % \begin{subfigure}[t]{0.155\textwidth}
    %     \includegraphics[width=\textwidth, height=2.5 cm]{Images/mafwat2.png}
    %     % No caption for Image 3
      
    % \end{subfigure}
    % \begin{subfigure}[t]{0.155\textwidth}
    %     \includegraphics[width=\textwidth, height=2.5 cm]{Images/maf2.png}
    %     % No caption for Image 4
        
    % \end{subfigure}\\
    \vspace{-0.01 em}

    \begin{subfigure}[t]{0.155\textwidth}
        \includegraphics[width=\textwidth, height=2.5 cm]{Images/gt.png}
        \caption{GT}
        \label{f3a}
    \end{subfigure}
    \begin{subfigure}[t]{0.155\textwidth}
        \includegraphics[width=\textwidth, height=2.5 cm]{Images/source_only.png}
        \caption{Source-only}
        \label{f3b}
    \end{subfigure}
    \begin{subfigure}[t]{0.155\textwidth}
        \includegraphics[width=\textwidth, height=2.5 cm]{Images/at2.png}
        \caption{AT~\cite{li2022cross} }
        \label{f3c}
    \end{subfigure}
    \begin{subfigure}[t]{0.155\textwidth}
        \includegraphics[width=\textwidth, height=2.5 cm]{Images/baseline.png}
        \caption{MRT~\cite{zhao2023masked}}
        \label{f3d}
    \end{subfigure}
    \begin{subfigure}[t]{0.155\textwidth}
        \includegraphics[width=\textwidth, height=2.5 cm]{Images/mafwat.png}
        \caption{\textbf{w/o ACR}}
        \label{f3e}
    \end{subfigure}
    \begin{subfigure}[t]{0.155\textwidth}
        \includegraphics[width=\textwidth, height=2.5 cm]{Images/maf.png}
        \caption{\textbf{Ours}}
        \label{f3f}
    \end{subfigure}
    \caption{Qualitative ablation: pseudo label analysis for In-house to INBreast.}
    \label{f3}
\end{figure}


==> tables/table-ablation.tex <==

\begin{table*}[t]
\caption{
	\textbf{Left:} Demonstrating superiority of our approach for natural image setting with \texttt{Sim10K}~\cite{johnson2016driving} as the source, and \texttt{Cityscapes}~\cite{cordts2016cityscapes} as the target dataset.
	\textbf{Right:} Comparing object detectors proposed for natural images with our method.  
}
\vspace{0.2em}
\centering
\label{ablation}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}l|l|ccc|c|ccl|l|c@{}}

         \cline{1-7} \cline{9-11}
%         \vspace{0.1cm}
        \makecell[c]{\textbf{Detector}} & \makecell[c]{\textbf{Venue}}  & \textbf{R@0.1} & \textbf{R@0.3} & \textbf{R@0.5}  & \hspace{0.1 cm}\textbf{Acc} \hspace{0.1 cm} & \hspace{0.1 cm}\textbf{F1} & \hspace{0.5cm}  & \makecell[c]{\textbf{Detector}} & \makecell[c]{\textbf{Venue}} & \textbf{AP(car)}
        \\
        \cline{1-7} \cline{9-11}
        FRCNN~\cite{ren2015faster} & NIPS'15   & 0.25 & 0.40 & 0.45 & 0.828 &0.297&  &FRCNN~\cite{ren2015faster}     & NIPS'15            & 39.4    \\
        YOLO-v5~\cite{ge2021yolox}& ICCVW’21    & 0.26 & 0.34 & 0.36 & 0.828 & 0.311& &SSAL~\cite{munir2021ssal} & NIPS'21        & 42.5         \\
        Cond.DETR~\cite{ge2021yolox} & ICCV’21  & 0.30 & 0.47 & 0.51  &0.833  &0.430 & &DA-Faster~\cite{chen2018domain}        & CVPR'18            & 41.9 \\   
        Dab-DETR~\cite{liu2022dab} & ICLR’22   & 0.43 & 0.57 & 0.63  & 0.843 &0.552 & & MeGACDA~\cite{vs2021mega}        & CVPR'21            & 44.8 \\   
        Dab DEF~\cite{liu2022dab}  & ICLR’22   & 0.40 & 0.46 & 0.50  & 0.830 & 0.546&& ViSGA~\cite{rezaeianaran2021seeking}            & ICCV'21            & 49.3 \\
        DN-DETR~\cite{li2022dn} & CVPR’22  & 0.38 & 0.47 & 0.58  & 0.828 & 0.393& &AQT~\cite{huang2022aqt} & IJCAI 2022          & 53.4          \\
        DN DEF.~\cite{li2022dn} & CVPR’22  & 0.39 & 0.44 & 0.47  & 0.825 & 0.526& &DA-Detr~\cite{zhang2023detr}   & CVPR'23          & 54.7        \\
        YOLO-V8~\cite{jocher2023yolo} & UT’23  & 0.06 & 0.08 & 0.10  & 0.258 &0.346 & & KTNet~\cite{tian2021knowledge}            & ICCV'21            & 50.7  \\
        FocalNET~\cite{yang2022focal} & NIPS’23   & 0.56 & 0.73 & 0.75  & 0.865 &0.641& &ConfMix~\cite{mattolin2023confmix} & CVPR'23          & 56.3       \\
        DINO~\cite{zhang2023dino} & ICLR’23   & 0.35 & 0.54 & 0.65 & 0.820 & 0.275& &PT~\cite{chen2022learning}               & PMLR'22            & 55.1  \\            
% \cline{1-7} \cline{9-11}
        \textbf{Ours} &  - & \textbf{0.53} & \textbf{0.71}  & \textbf{0.75}  & \textbf{0.879} &  \textbf{0.773}& & \textbf{Ours}  & -          & \textbf{59.1}        \\
        \cline{1-7} \cline{9-11}
    \end{tabular}%
\end{adjustbox}

\end{table*}

==> tables/table2.tex <==
\begin{table}[t]
\centering
\resizebox{\textwidth}{!}{%
	\setlength{\tabcolsep}{6pt}
\begin{tabular}{c|c|c|c|cccccc}
\hline
\textbf{Source} & \textbf{AT~\cite{li2022cross}} & \textbf{MA} & \textbf{ACR} & \textbf{R@0.025} & \textbf{R@0.05} & \textbf{R@0.1} & \textbf{R@0.3} & \textbf{R@0.5} & \textbf{R@0.9} \\
\hline
\checkmark & & & & 0.19 & 0.34 & 0.43 & 0.57 & 0.65 & 0.69 \\
\checkmark & & \checkmark & & \textbf{0.39} & 0.46 & 0.53 & 0.71 & 0.75 & 0.78 \\
\checkmark & \checkmark & & & 0.28 & 0.35 & 0.42 & 0.61 & 0.64 & 0.69 \\
\checkmark & \checkmark & & \checkmark & 0.30 & 0.42 & 0.51 & 0.61 & 0.70 & 0.71 \\
\checkmark & \checkmark & \checkmark & & 0.37 & 0.46 & 0.59 & 0.72 & 0.75 & 0.75 \\
\checkmark & \checkmark & \checkmark & \checkmark & \textbf{0.39} & \textbf{0.51} & \textbf{0.53} & \textbf{0.71} & \textbf{0.75} & \textbf{0.79} \\
\hline
\end{tabular}
}%
\\ \vspace{0.5em}\begin{tabular}{cccccc}
\includegraphics[width=0.158\textwidth, height= 2.7 cm]{Images/S_FINAL.png}
&
\includegraphics[width=0.158\textwidth, height= 2.7 cm]{Images/SMA_FINAL.png}
&
\includegraphics[width=0.158\textwidth, height= 2.7 cm]{Images/AT_FINAL.png}
&
\includegraphics[width=0.158\textwidth, height= 2.7 cm]{Images/AT_ACR_FINAL.png}
&
\includegraphics[width=0.158\textwidth, height= 2.7 cm]{Images/AT_MA_FINAL.png}
&
\includegraphics[width=0.158\textwidth, height= 2.7 cm]{Images/MAF_FINAL.png}
\end{tabular}
\caption{\textbf{Ablation study to understand impact of each proposed module for In-house to \inbreast adaptation.} ``Source'' denotes the source-only trained model, ``Baseline'' the basic teacher-student architecture, ``MA'' the proposed mask annealing technique, and ``ACR'' denotes adaptive confidence refinement module. The figures from left to right correspond to qualitative results from row 1 to row 6 respectively. Red boxes denote the ground truth, and blue boxes show the predicted regions.}
\label{tab:ablation}
\end{table}



==> tables/table3.tex <==
    \begin{table}[H]
        \begin{minipage}{0.65\textwidth}
            \begin{minipage}{0.50\textwidth}
                \centering
                \begin{subtable}{\textwidth}
                    \centering
                    \caption{Mask Ratio}
                    \begin{tabular}{cc}
                        \toprule
                        Mask Ratio & R@0.3 \\
                        \midrule
                        0.3   & \textbf{0.61}  \\
                        0.5   & 0.57  \\
                        0.8  & 0.44   \\
                        % Add more rows as needed
                        \bottomrule
                    \end{tabular}
                \end{subtable}
                
                \begin{subtable}{\textwidth}
                    \centering
                    \caption{Coefficient Decay}
                    \begin{tabular}{cc}
                        \toprule
                        Strategy & R@0.3 \\
                        \midrule
                        No decay   & 0.65   \\
                        Linear   & 0.72   \\
                        Hard   & \textbf{0.74}   \\
                        % Add more rows as needed
                        \bottomrule
                    \end{tabular}
                \end{subtable}
                
                
               
            \end{minipage}%
            \begin{minipage}{0.50\textwidth}
                \centering
                \begin{subtable}{\textwidth}
                    \centering
                    \caption{Training Data}
                    \begin{tabular}{cc}
                        \toprule
                        Training Data & R@0.3 \\
                        \midrule
                        Source   & 0.63 \\
                        Target   &  0.71 \\
                        Source and Target & \textbf{0.74}  \\
                        % Add more rows as needed
                        \bottomrule
                    \end{tabular}
                \end{subtable}
                 
                \begin{subtable}{\textwidth}
                    \centering
                    \caption{Annealing}
                    \begin{tabular}{cc}
                        \toprule
                        Annealing  & R@0.3 \\
                        \midrule
                        Step   & 0.   \\
                        Cyclic   & 0.71   \\
                        Cosine  & \textbf{0.74}   \\
                        % Add more rows as needed
                        \bottomrule
                    \end{tabular}
                \end{subtable}
            
    
    
                
            \end{minipage}
        \end{minipage}%
        \begin{minipage}{0.35\textwidth}
            \centering
            
            \includegraphics[width=\textwidth]{Images/T-sne_before.png} \\
            \includegraphics[width=\textwidth]{Images/T-sne_after.png}
            \label{fig:figure1and2}
        \end{minipage}
        \caption{ \small{The MAE ablation study revealed key insights: starting with a low mask ratio enhances self-supervised tasks, decay in $\lambda_{mask}$ boosts performance, training on both source target features encodes better features and D-MASTER approach mitigates overfitting compared to traditional methods}}
    \end{table}

==> tables/table4.tex <==
\begin{table}[htbp]
    \centering
    \caption{Results of Sim10k to Cityscapes(car) showcasing our proposed mask annealing works better in similar natural image setting}
    \label{tab:method_comparison}
    \begin{tabular}{@{}p{0.19\textwidth}p{0.16\textwidth}c@{\hspace{0.05\textwidth}}}
        \toprule
        \textbf{Method} & \textbf{Venue} & \textbf{carAP} \\ 
        \midrule
        FRCNN~\cite{ren2015faster}     & NIPS'15            & 39.4    \\    SSAL~\cite{munir2021ssal} & NIPS'21        & 42.5         \\
        DA-Faster~\cite{chen2018domain}        & CVPR'18            & 41.9 \\      
        MeGACDA~\cite{vs2021mega}        & CVPR'21            & 44.8 \\  
    ViSGA~\cite{rezaeianaran2021seeking}            & ICCV'21            & 49.3 \\ 
         AQT~\cite{huang2022aqt} & IJCAI 2022          & 53.4          \\
  DA-Detr~\cite{zhang2023detr}   & CVPR'23          & 54.7        \\
        KTNet~\cite{tian2021knowledge}            & ICCV'21            & 50.7          \\ConfMix~\cite{mattolin2023confmix} & CVPR'23          & 56.3       \\
        PT~\cite{chen2022learning}               & PMLR'22            & 55.1  \\           \textbf{Ours}  & -          & \textbf{59.1}        \\
        \bottomrule
    \end{tabular}
    \label{t5}
\end{table}




==> tables/table5.tex <==
\begin{table}[htbp]
    \centering
    \small
    \caption{Comparison of state-of-the-art object detectors with our method.}
    \label{tab:method_comparison}
    \begin{tabular}{@{}l|c|ccccc|c|c@{}}
        \toprule
        \textbf{Detector} & \textbf{Venue} & \textbf{R@0.025} & \textbf{R@0.1} & \textbf{R@0.3} & \textbf{R@0.5} & \textbf{R@1} & \textbf{Accur} & \textbf{F1-Score} \\
        \midrule
        FRCNN~\cite{ren2015faster} & NIPS'15  & 0.16 & 0.25 & 0.40 & 0.45 & 0.54 & 0.828 &0.297 \\
        YOLO-v5~\cite{ge2021yolox}& ICCVW’21   & 0.19 & 0.26 & 0.34 & 0.36 & 0.44 & 0.828 & 0.311\\
        Cond.DETR~\cite{ge2021yolox} & ICCV’21  & 0.15 & 0.30 & 0.47 & 0.51 & 0.60 &0.833  &0.430 \\
        Dab-DETR~\cite{liu2022dab} & ICLR’22  & 0.20 & 0.43 & 0.57 & 0.63 & 0.72& 0.843 &0.552 \\
        Dab DEF~\cite{liu2022dab}  & ICLR’22  & 0.10 & 0.40 & 0.46 & 0.50 & 0.55 & 0.830 & 0.546\\
        DN-DETR~\cite{li2022dn} & CVPR’22 & 0.19 & 0.38 & 0.47 & 0.58 & 0.62 & 0.828 & 0.393\\
        DN DEF.~\cite{li2022dn} & CVPR’22 & 0.17 & 0.39 & 0.44 & 0.47 & 0.51 & 0.825 & 0.526\\
        YOLO-V8~\cite{jocher2023yolo} & UT’23 & 0.02 & 0.06 & 0.08 & 0.10 & 0.12 & 0.258 &0.346 \\
        FocalNET~\cite{yang2022focal} & NIPS’23  & 0.28 & 0.56 & 0.73 & 0.75 & \textbf{0.82} & 0.865 & 0.641\\
        DINO~\cite{zhang2022dino} & ICLR’23  & 0.20 & 0.35 & 0.54 & 0.65 & 0.75 & 0.820 & 0.275\\
        
        \midrule
        \textbf{Ours} &  & \textbf{0.39} & \textbf{0.60} & \textbf{0.74}  & \textbf{0.76} & 0.78 & \textbf{0.879} &  \textbf{0.773}\\
        \bottomrule
    \end{tabular}
    \label{t4}
\end{table}


==> tables/table6.tex <==
\begin{table}[H]
    \centering
    \caption{Below are the detailed hyper-parameters corresponding to each benchmark, with the source dataset as the In-house dataset}
    \label{tab:implementation_details}
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{@{}clcc@{}}
        \toprule
        \textbf{Hyper-parameter} & \textbf{Description} & \textbf{INBreast} & \textbf{DDSM}  \\
        \midrule
       $N_c$ & Number of categories for classification head  & 2 & 2  \\
        $N_l^{\text{enc}}$& Number of encoder layers  & 8 & 6  \\
        $N_l^{\text{dec}}$ & Number of decoder layers   & 8 & 6   \\
        $N_l^{\text{aux}}$ &Number of MAE auxiliary decoder layers  & 2& 2  \\
        $N_q^{\text{dec}}$ & Number of queries for decoder   & 300 & 300 \\
        $N_q^{\text{aux}}$ &Number of queries for MAE auxiliary decoder & 882  & 882\\
        $H$& Number of hidden dimension for deformable attention& 256 &  256\\
        $F$ & Number of feedforward dimension for deformable attention   & 1024 &1024 \\
        $L$ & Number of feature levels for deformable attention   & 4& 4  \\
        $M$ & Number of heads for deformable attention & 8& 8\\
        $K$ & Number of reference points for each attention head& 4 & 4 \\
        % $dropout$& Ratio for dropout in Deformable DETR   & 0.0& 0.0 & 0.0\\
        $B$ & Batch Size during training   & 16 &16   \\
        $lr$ & Learning rate for modules except backbone and projection   & $2 \times 10^{-4}$&$ 2 \times 10^{-4}$\\
        $lr_{bac}$ & Learning rate for backbone and projection modules   & $2 \times 10^{-5}$ & $2 \times 10^{-5}$ \\
        $\beta_{bac}$ & Coefficient of discrimination loss after backbone $L_{\text{bac}}^{\text{dis}}$& 0.3 & 0.3 \\
        $\beta_{enc}$ & Coefficient of discrimination loss after encoder $L_{\text{enc}}^{\text{dis}}$
 & 1.0 &  1.0 \\
        $\beta_{dec}$ &Coefficient of discrimination loss after decoder $L_{\text{enc}}^{\text{dis}}$
 &  1.0 &  1.0 \\
        $\lambda_{unsup}$ & Coefficient of unsupervised loss $\mathcal{L}_{unsup}$ &  1.0 &  1.0 \\
        $\lambda_{mask}$ & Coefficient of supervised loss $\mathcal{L}_{sup}$ &  1.0 &  1.0\\
        $\gamma$ & EMA update ratio & 0.9996 & 0.9996 \\
        $\mu_{t}$ & Initial Mask ratio in MAE branch & 0.2 & 0.3 \\
        $\eta$ & Initial step for annealing & 0.2 & 0.3 \\

        $\eta^i_{min}$ & Minimum jump in mask annealing step $\eta$ & 0.05 & 0.05 \\
        $\eta^i_{max}$ & Maximum jump in mask annealing step $\eta$ & 0.15 & 0.15 \\
        $C_s$&Soft Confidence Metric&0.15&0.20\\
        $C_h$&Hard Confidence Metric&0.80&0.90\\\
        $E_{pre}$ & MAE branch with source data training epoch number & 88 & 87  \\
        $E_{teach}$ & Teacher-student training epoch number & 84 & 76 \\
        $E_{decay}$ & After Edecay epochs in teaching stage, we drop the MAE branch & 30 & 10\\
        $E_{reinit}$ & Re-initialization epoch for selective retraining & 40 & 20 \\
        
        \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table}


==> tables/table7.tex <==
\begin{table*}[hbtp]
\centering
  \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}c|l|l|cccccc|cc@{}}
    \toprule
    \textbf{Datasets}& \makecell[c]{\textbf{Model Name}} & \makecell[c]{\textbf{Venue}} & \textbf{R@0.05} & \textbf{R@0.1} & \textbf{R@0.3} &\textbf{R@0.5}& \textbf{R@1.0} & \textbf{R@2.0} & \textbf{Accuracy} & \textbf{F1-score} \\ \midrule
    & SFA\cite{wang2021exploring} & MM'21&0.01 & 0.01& 0.05& 0.07& 0.11&0.313 & 0.216&0.329\cr
    & UMT\cite{deng2021unbiased} & CVPR'21 &0.0 & 0.01&0.04 & 0.07& 0.09&0.13 & 0.261&0.362\cr
    & D-Adapt\cite{jiang2021decoupled} & ICLR'22 &0.0 & 0.02& 0.06&0.09 &0.10 &0.13 &0.382 &0.215\cr
    & AT\cite{li2022cross} & CVPR'22 & 0.01& 0.03&0.08 &0.10 &0.15 & 0.21&0.216 & 0.311\cr
    \textbf{\texttt{In-house} to} & H2FA\cite{xu2022h2fa} & CVPR'22 &0.02 & 0.03&0.06 &0.10 & 0.12&0.17 &0.371&0.315 \cr
    \textbf{\ddsm~\cite{lee2017curated}} & AQT\cite{huang2022aqt} & IJCAI'22 &0.01 &0.03 & 0.07& 0.13& 0.15&0.18 &0.412&0.398\cr
    & HT\cite{deng2023harmonious}  & CVPR'23 & 0.03&0.05&0.08 &0.10 &0.13 & 0.15&0.362&0.362 \cr
    & ConfMIX\cite{mattolin2023confmix} & WACV'23& 0.02&0.04 &0.09 &0.12 &0.16 &0.19 &0.336 &0.412\cr
    & CLIPGAP\cite{vidit2023clip} & CVPR'23 &0.01& 0.03& 0.07& 0.11& 0.15& 0.16& 0.336& 0.458\cr
    & MRT\cite{zhao2023masked} & ICCV'23 &0.03& 0.04& 0.09&0.12 & 0.17& 0.21&0.421 &0.587 \cr
    & \textbf{Ours} &- & \textbf{0.02}& \textbf{0.05} & \textbf{0.12} & \textbf{0.17} & \textbf{0.29} & \textbf{0.49}&\textbf{0.561}&\textbf{0.613} \cr \midrule
    & SFA\cite{wang2021exploring} & MM'21& 0.03& 0.07&0.13 &0.18 & 0.27&0.31& 0.629&0.210\cr
    & UMT\cite{deng2021unbiased} & CVPR'21  & 0.01&0.04& 0.09&0.15 &0.19 &0.23 &0.568&0.193\cr
    & D-Adapt\cite{jiang2021decoupled} & ICLR'22&0.03 &0.06 & 0.11& 0.18&0.25 &0.31 &0.668&0.241 \cr
    & AT\cite{li2022cross} & CVPR'22  & 0.10&0.28& 0.37& 0.45& 0.51& 0.66&0.725&\textbf{0.319}\cr
    \textbf{\rsna to} & H2FA\cite{xu2022h2fa} &CVPR'22& 0.03& 0.06& 0.14& 0.17&0.21 & 0.24& 0.591&0.274 \cr
    \textbf{\texttt{In-house}} & AQT\cite{huang2022aqt} &IJCAI'22&0.01 &0.05 &0.08 & 0.11& 0.17& 0.20& 0.527&0.230 \cr
    & HT\cite{deng2023harmonious}  & CVPR'23 &0.02& 0.10& 0.17&0.24 &0.33 & 0.41& 0.710&0.291\cr
    & ConfMIX\cite{mattolin2023confmix} & WACV'23 &0.03& 0.09&.0.16 &0.28 & 0.35& 0.39& 0.622&0.263 \cr
    & CLIPGAP\cite{vidit2023clip} & CVPR'23 &0.04& 0.08&0.23 & 0.36&0.64 &0.72 & 0.797&0.231\cr
    & MRT\cite{zhao2023masked} & ICCV'23 &0.06 & 0.11&0.29 &0.44 & 0.65&0.76 & 0.825& 0.304\cr
    & \textbf{Ours} & &  \textbf{0.14} & \textbf{0.20} & \textbf{0.37} & \textbf{0.54} & \textbf{0.72} & \textbf{0.83} & \textbf{0.825}&0.312 \cr \bottomrule
    \end{tabular}
  }
  \vspace{0.2em}
  \caption{\cref{tab:sota_uda_comparison} in the main paper showed similar comparison with \sota \uda methods on few dataset pairs. Here we show results for few more pairs.}
  \label{tab:sota_uda_comparison_suppl}


\end{table*}

==> tables/table8.tex <==


\begin{figure}[htbp]
\centering
\begin{subfigure}[b]{0.15\textwidth}
  {\centering\caption{\texttt{In-house}}}
  \vspace{0.95cm}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[height=2.1cm, width= 2 cm]{Images/aiims_Source.png}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[height=2.1cm, width= 2 cm]{Images/aiims_AT.png}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[height=2.1cm, width= 2 cm]{Images/aiims_mrt.png}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[height=2.1cm, width= 2 cm]{Images/aiims_ht.png}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[height=2.1cm, width= 2 cm]{Images/aiims_ours.png}
\end{subfigure}
\vspace{-0.02em}
\begin{subfigure}[b]{0.15\textwidth}
  {\centering\caption{\ddsm~\cite{lee2017curated}}}
  \vspace{0.95cm}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[height=2.1cm, width= 2 cm]{Images/ddsm_S.png}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[height=2.1cm, width= 2 cm]{Images/ddsm_AT.png}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[height=2.1cm, width= 2 cm]{Images/ddsm_mrt.png}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[height=2.1cm, width= 2 cm]{Images/ddsmht.png}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[height=2.1cm, width= 2 cm]{Images/ddsm_ours.png}
\end{subfigure}
\vspace{-0.01em}
\begin{subfigure}[b]{0.15\textwidth}
  {\centering\caption{\rsna}}
  \vspace{1.55cm}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[height=2.1cm, width=2cm]{Images/rsna_s.png}
    \caption{Source}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[height=2.1cm, width=2cm]{Images/rsna_at.png}
    \caption{AT~\cite{li2022cross}}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[height=2.1cm, width=2cm]{Images/rsna_mrt.png}
    \caption{MRT~\cite{zhao2023masked}}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[height=2.1cm, width=2cm]{Images/rsna_ht.png}
    \caption{HT~\cite{deng2023harmonious}}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.16\textwidth}
    \includegraphics[height=2.1cm, width=2cm]{Images/rsna_ours.png}
    \caption{Ours}
\end{subfigure}
\caption{Qualitative result comparison on in-house, \ddsm, and \rsna datasets. Red boxes show the ground truth, and blue boxes show the predictions.}
\label{fig:qualitative_results}
\end{figure}


==> tables/table9.tex <==
\begin{table*}[t]
\centering
\begin{minipage}[b]{0.68\linewidth} % Adjust the width as needed
\resizebox{\linewidth}{!}
{
\begin{tabular}{@{}c|c|c|cccccc@{}}
\toprule
\textbf{Datasets}& \textbf{Model Name} & \textbf{Venue} & \textbf{R@0.025} & \textbf{R@0.1} & \textbf{R@0.3} & \textbf{R@0.5}& \textbf{R@1} & \textbf{R@2}   
\\ 
\midrule
& SFA\cite{wang2021exploring} & ACM-M'21 &0.02 &0.09 & 0.16& 0.19& 0.24&0.31 
\\
& UMT\cite{deng2021unbiased} & CVPR'21 &0.04 &0.12 & 0.16&0.23 &0.32 & 0.38 
\\
& D-Adapt\cite{jiang2021decoupled} & ICLR'22 &0.09 &0.15 &0.21& 0.26 & 0.35&0.43  
\\
& AT\cite{li2022cross} & CVPR'22 & 0.08& 0.16& 0.28& 0.35& 0.56&0.79  
\\
\textbf{DDSM to} & H2FA\cite{xu2022h2fa} & CVPR'22 &0.02 &0.08 & 0.16& 0.21& 0.28& 0.37
\\
\textbf{In-house} & AQT\cite{huang2022aqt} & IJCAI'22 & 0.01&0.08 & 0.15& 0.19&0.28&0.33 
\\
& HT\cite{deng2023harmonious}  & CVPR'23 &0.09 & 0.18&0.28&  0.31& 0.38& 0.46
\\
& ConfMIX\cite{mattolin2023confmix} & WACV'23 & 0.05& 0.09& 0.14&0.19& 0.29& 0.37 
\\
& CLIPGAP\cite{vidit2023clip} & CVPR'23 & 0.08& 0.19& 0.29& 0.38& 0.58& 0.81
\\
& MRT\cite{zhao2023masked} & ICCV'23 & 0.03 & 0.14 & 0.27&  0.35&0.58   &  0.67
\\
& \textbf{Ours} & & \textbf{0.15} & \textbf{0.34} & \textbf{0.49} & \textbf{0.61}& \textbf{0.76} & \textbf{0.88} 
\\ 
\bottomrule
\end{tabular}
}
\caption{Results of DDSM to In-house dataset.}
\label{t2a}
\end{minipage}
\hfill
\begin{minipage}[b][\totalheight][b]{0.3\linewidth} % Adjust the width as needed
  \centering
\includegraphics[width=\textwidth, height= 3.5 cm]{Images/In-house.png}\\
  \captionof{figure}{FROC curve}
  \label{t2b}
\end{minipage}
\end{table*}
